A fast and spectrally convergent algorithm for rational-order fractional integral and differential equations

A fast algorithm (linear in the degrees of freedom) for the solution of linear variable-coefficient rational-order fractional integral and differential equations is described. The approach is related to the ultraspherical method for ordinary differential equations [Olver & Townsend 2013], and involves constructing two different bases, one for the domain of the operator and one for the range of the operator. The bases are constructed from direct sums of suitably weighted ultraspherical or Jacobi polynomial expansions, for which explicit representations of fractional integrals and derivatives are known, and are carefully chosen so that the resulting operators are banded or almost-banded. Geometric convergence is demonstrated for numerous model problems when the variable coefficients and right-hand side are sufficiently smooth.

==> extensions_old.tex <==
\subsection{Extensions 1: Nonlinear problems}\label{sec:nonlin}\cite{levinson1960}\\
\includegraphics[width=300pt]{figures/nonlin}\\
\includegraphics[width=300pt]{figures/nonlin_soln}

\subsection{Extensions 2: Time dependent problems}\label{sec:time}
\begin{figure}\label{fig:fracdiff}
\centering\tiny
\includegraphics[height=110pt]{figures/waterfall}
\caption{Numerical solution to~(\ref{eqn:fracadvdiff}) using the trapezium rule in time with $h = 0.0001$ and $n = 200$ coefficients in space.
}
\end{figure}


A natural application of the approach is to time-evolution equations, for example, a fractional advection--diffusion equation
%
\begin{equation}\label{eqn:fracadvdiff}
u_t = u_{xx} + \prescript{RL\!}{-1}{\calD}_x^{1/2}u
\end{equation}
%
with initial condition $u(0,x) = u_0(x)$ and Dirichlet boundary conditions $u(t,-1) = u(t,1) = 0$.   As a simple example, one can perform a Trapezoidal rule discretization, resulting in a sequence of fractional differential equations:
%
	$$[I - h/2 ({\cal D}^2 + \prescript{RL\!}{-1}{\calD}_x^{1/2})] u_{k+1} = u_k + h/2 ({\cal D}^2 + \prescript{RL\!}{-1}{\calD}_x^{1/2}) u_k.$$
%
We discretize the fractional differential operator by representing its action on $n=200$ coefficients in the proposed sum space basis, that is, 100 coefficients in each component, and take $h=0.0001$, see Figure~\ref{fig:fracdiff}. 

%While this example problem has been successfully solved, there are numerous outstanding issues.  
